MCRB-based Performance Analysis of 6G Localization under Hardware Impairments

Location information is expected to be the key to meeting the needs of communication and context-aware services in 6G systems. User localization is achieved based on delay and/or angle estimation using uplink or downlink pilot signals. However, hardware impairments (HWIs) distort the signals at both the transmitter and receiver sides and thus affect the localization performance. While this impact can be ignored at lower frequencies where HWIs are less severe, modeling and analysis efforts are needed for 6G to evaluate the localization degradation due to HWIs. In this work, we model various types of impairments and conduct a misspecified Cram\'er-Rao bound analysis to evaluate the HWI-induced performance loss. Simulation results with different types of HWIs show that each HWI leads to a different level of degradation in angle and delay estimation performance.

==> IEEEabrv.tex <==


IEEE Journals


aerospace and military
@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV         = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE        = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}



circuits, signals, systems, audio and controls
@STRING{IEEE_J_STSP       = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST       = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
in 2014 ASL became ASLP
@STRING{IEEE_J_ASLP       = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL        = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP    = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB   = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS      = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}



communications
@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML      = "{IEEE} Wireless Commun. Lett."}



components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
in 2011 CAPT became CPMT
@STRING{IEEE_J_CPMT       = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART      = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



CAD
@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}



coding, data, information, knowledge
@STRING{IEEE_J_BD         = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS        = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}



computers, computation, networking and software
@STRING{IEEE_J_CAL        = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES         = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT        = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC       = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT       = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC       = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC         = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS        = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS        = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC        = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC        = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS       = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE        = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM        = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
in 2012 NN became NNLS
@STRING{IEEE_J_NNLS       = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC         = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN       = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}



computer graphics, imaging, and multimedia
@STRING{IEEE_J_JDT        = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}



cybernetics, ergonomics, robots, man-machine, artificial intelligence and automation
@STRING{IEEE_J_JAS        = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC       = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE        = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD        = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN        = "{IEEE} Trans. on Cogn. Commun. Netw."}
in 2015 AMD became CDS
@STRING{IEEE_J_CDS        = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG      = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
in 2013 SMCB became CYB
@STRING{IEEE_J_CYB        = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H          = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
in 2013 SMCC became HMS
@STRING{IEEE_J_HMS        = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
in 1989 JRA became RA
in August 2004, RA split into ASE and RO
@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL        = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO         = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
in 2012 SMCA became SMCS
@STRING{IEEE_J_SMCS       = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}



earth, wind, fire and water
@STRING{IEEE_J_GRSL       = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE         = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS      = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}



education, engineering, history, IEEE, professional
@STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA       = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT         = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL       = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL       = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL       = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC       = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID       = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ       = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



energy, power and conversion
@STRING{IEEE_J_PHOT       = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL        = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS       = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE      = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG         = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE        = "{IEEE} Trans. Sustain. Energy"}



industrial, commercial and consumer
@STRING{IEEE_J_PSE        = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF       = "{IEEE} Trans. Ind. Informat."}



instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



insulation and materials
@STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI         = "{IEEE} Trans. Electr. Insul."}



mechanical
@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}
in 2014 MEMS became MEMSI
@STRING{IEEE_J_MEMSI      = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatronics"}



medical and biological
@STRING{IEEE_J_BHI        = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM       = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS         = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME       = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS       = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
B-ME later dropped the hyphen and became the BME
@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB        = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC       = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehabil. Eng."}



optics, lightwave and photonics
@STRING{IEEE_J_JLT        = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN        = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ         = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}



physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS        = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO      = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



reliability
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



semiconductors, superconductors, electrochemical and solid state
@STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM         = "{IEEE} Trans. Semicond. Manuf."}



sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}





IEEE Magazines and Online Publications


@STRING{IEEE_O_ACC        = "{IEEE} Access"}
@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST       = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC     = "China Commun."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO       = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM        = "{IEEE} Comput. Intell. Mag."}
CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C          = "Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
in 2012 DTC became DT
@STRING{IEEE_M_DT         = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO        = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF        = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC        = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_GRS        = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE         = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS        = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO       = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET        = "{IEEE} Netw."}
IEEE's editorial manual lists "Pers. Commun.",
but "Personal Commun. Mag." seems to be what is used in the journals
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC        = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL        = "{IEEE} Power Electron. Mag."}
CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE      = "{IEEE} Pulse"}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP        = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."}
@STRING{IEEE_M_SSC        = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC        = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT         = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY      = "Today's Engineer"}

% Journal
% COMST:IEEE Commun. Surveys Tuts.
% TSP:  IEEE Trans. Signal Process.
% TWC:  IEEE Trans. Wireless Commun.
% TCOM: IEEE Trans. Commun.
% JSAC: IEEE J. Sel. Areas Commun.
% JSTSP:IEEE J. Sel. Topics Signal Process.
% ISJ:  IEEE Syst. J.
% ITS:  IEEE Trans. Intell. Transp. Syst.
% MTT:  IEEE Trans. Microw. Theory Techn.
% TMC:  IEEE Trans. Mobile Comput.
% TIM:  IEEE Trans. Instrum. Meas.


% Letter 
% WCL:  IEEE Wireless Commun. Lett.
% Magazine
% SP magazine: IEEE Signal Process. Mag.
% Com mag.
% Open Journal
% OJ-COMS: IEEE Open J. Commun. Soc.
% OJVT: IEEE Open J. Veh. Technol.

% Conf.
% EuCAP:    Proc. Eur. Conf. Antennas Propag. (EuCAP)
% GLOBECOM: Proc. IEEE Global Commun. Conf. (GLOBECOM)
% ICASSP:   Proc. IEEE Int. Conf. Acoust., Speech, Signal Process. (ICASSP)
% ICC:      Proc. IEEE Int. Conf. Commun. (ICC)
% VTC:      IEEE Veh. Technol. Conf. (VTC)
% WCNC:     Proc. IEEE Wireless Commun. Netw. Conf. (WCNC)
% PIMRC:    Proc. Annu. Int. Symp. Pers. Indoor Mobile Radio Commun. (PIMRC)
% InfoCOM:  Proc. IEEE Conf. Comput. Commun. (INFOCOM)
% EUCNC:    Eur. Conf. Netw., Commun. (EuCNC)
--
EOF


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

